Presburger arithmetic with threshold counting quantifiers is easy

We give a quantifier elimination procedures for the extension of Presburger arithmetic with a unary threshold counting quantifier $\exists^{\ge c} y$ that determines whether the number of different $y$ satisfying some formula is at least $c \in \mathbb N$, where $c$ is given in binary. Using a standard quantifier elimination procedure for Presburger arithmetic, the resulting theory is easily seen to be decidable in 4ExpTime. Our main contribution is to develop a novel quantifier-elimination procedure for a more general counting quantifier that decides this theory in 3ExpTime, meaning that it is no harder to decide than standard Presburger arithmetic. As a side result, we obtain an improved quantifier elimination procedure for Presburger arithmetic with counting quantifiers as studied by Schweikardt [ACM Trans. Comput. Log., 6(3), pp. 634-671, 2005], and a 3ExpTime quantifier-elimination procedure for Presburger arithmetic extended with a generalised modulo counting quantifier.

==> lower-bounds.tex <==
\section{Lower bounds}
\label{section:lower-bounds}

\todo[inline]{todo}

==> quantifier-elimination-variants.tex <==
\section{Eliminating other counting quantifiers}
\label{section:quantifier-elimination-variants}

In this section, we extend the quantifier-elimination procedure introduced in~\Cref{section:quantifier-elimination} in order to eliminate the counting quantifiers~$\exists^{\geq c}\avarbis$, ~$\exists^{= \avar}\avarbis$, and~$\exists^{(\avar,q)}\avarbis$.

\subsection{Elimination of a threshold counting quantifier}
\label{subsection:elimination-treshold-quantifiers}

Consider a formula~$\Aformula_0 = \exists^{\geq c}\avarbis\,\aformula$ with $\varphi$ quantifier free.
%% , where $\aformula$ is a Boolean combination of linear inequalities and simple modulo constraints.
By definition,~$\Aformula_0$ is equivalent to $\exists \avarter\,(\avarter = c \land \exists^{\geq \avarter} \avarbis\,\aformula)$ for some variable~$\avarter$ not occurring in~$\aformula$. Let $\Aformula_5$ be the formula obtained by performing the quantifier-elimination procedure of~\Cref{section:quantifier-elimination} on~$\exists^{\geq \avarter} \avarbis\,\aformula$, so that $\Aformula_0 \fequiv \exists \avarter\,(\avarter = c \land \Aformula_5) \fequiv \Aformula_5\substitute{\avarter}{c}$.
Recall that $\Aformula_5$ is defined as 
\begin{center}
$\Aformula_5 \egdef \bigvee_{i \in [1,o]}\bigvee_{r\colon Z\to [m]} (\Gamma_{i,r} \land \Aformula_5^{i,r})$.
\end{center}
Here, $Z = \vars{\aformula}$, $m = \lcm(\fmod{\Aformula_1})$ (defined as in the Step II of the procedure) and~$\Gamma_{i,r}$ is a conjunction of inequalities and simple modulo constraints with variables from~$Z$ 
(hence,~\mbox{$\avarter$-free}). 
Hence,~$\Gamma_{i,r}\substitute{\avarter}{c} = \Gamma_{i,r}$.
Moreover,~$\Aformula_5^{i,r}$ is either $\true$ or a formula of the form 
\begin{equation}
    \label{equation:5ir-form}
    m\avarter \leq p_2(t_{2}' - t_{1}') + r_2 + \dots + p_\ell(t_{\ell}' - t_{\ell-1}') + r_\ell + m(c_1 + \dots + c_\ell).
\end{equation}
where the terms $\aterm_1',\dots,\aterm_{\ell}'$ are from~$T \cup \{0\}$ (with~$T$ defined as in Step II of~\Cref{section:quantifier-elimination}), and thus written with variables from~$Z$. 
Therefore, the following property holds:
\begin{claim}
    \label{claim:zed-almost-free}
    In~$\Aformula_5$, $\avarter$ only appears on the left hand side of 
    inequalities of the form~\eqref{equation:5ir-form}. 
\end{claim}

We proceed with manipulating the disjuncts of~$\Aformula_5\substitute{\avarter}{c}$ separately.
Fix $i \in [1,o]$ and~${r \colon Z \to [m]}$. We aim at defining a formula~$\aformulater_{i,r}$ equivalent to the disjunct~$(\Gamma_{i,r} \land \Aformula_5^{i,r})\substitute{\avarter}{c}$ of $\Aformula_5\substitute{\avarter}{c}$.
\begin{itemize}
    \setlength{\itemsep}{2pt}
    \item If~$\Aformula_5^{i,r} = \true$, let $\aformulater_{i,r} \egdef \Gamma_{i,r}$.
    \item Else,~$\Aformula_5^{i,r}$ is as in~\eqref{equation:5ir-form}.
    Consider~$\Aformula_5^{i,r}\substitute{\avarter}{c}$, which is of the form 
    \begin{center}
        $m c \leq p_2(t_{2}' - t_{1}') + r_2 + \dots + p_\ell(t_{\ell}' - t_{\ell-1}') + r_\ell + m(c_1 + \dots + c_\ell)$.
    \end{center}
    By~\Cref{claim:zed-almost-free}, the occurrence of $c$ in the left side of this inequality is the only one introduced by the substitution $\substitute{\avarter}{c}$.
    \begin{itemize}
        \setlength{\itemsep}{3pt}
        \item Let $e = mc - (r_2 + \cdots + r_\ell + m(c_1+ \cdots + c_\ell))$.
        \item Let $I \subseteq \Nat^\ell$ be the set of tuples~$(i_2,\dots,i_\ell) \in [0,e]^{\ell}$ such that
          %(1) for every $j \in [2,\ell]$, if $p_j = 0$ then $i_j = 0$, and (2) 
        $e \leq i_2p_2 + \dots + i_\ell p_\ell$. 
        \item Let $\aformulater_{i,r} \egdef \Gamma_{i,r} \land \bigvee_{(i_2,\dots,i_\ell) \in I} \bigwedge_{j \in [2,\ell]} \aterm_j' - \aterm_{j-1}' \geq i_j$.
    \end{itemize}
\item Let $\Aformula_6^c = \bigvee_{i \in [1,o]}\bigvee_{r\colon Z\to [m]} \aformulater_{i,r}$. 
\end{itemize}
After defining~$\Aformula_6^c$, the procedure ends.
Notice that the inequalities~$\aterm_j' - \aterm_{j-1}' \geq i_j$ that replace the inequalities given in~\eqref{equation:5ir-form} are such that $\aterm_{j-1}',\aterm_{j}' \in T \cup \{0\}$. This leads to a better bound on the set~$\homterms{\Aformula_6^c}$, which 
ultimately enables us to establish the~\twoexpspace membership of Presburger arithmetic with threshold counting quantifiers.

\begin{restatable}{claim}{ClaimThresholdQEProcedure}
    $\Aformula_0 \fequiv \Aformula_6^c$. The formula $\Aformula_6^c$ is a Boolean combination of linear inequalities and simple modulo constraints.
\end{restatable}




